Can Large Language Models Grasp Concepts in Visual Content? A Case Study on YouTube Shorts about Depression

Large language models (LLMs) are increasingly used to assist computational social science research. While prior efforts have focused on text, the potential of leveraging multimodal LLMs (MLLMs) for online video studies remains underexplored. We conduct one of the first case studies on MLLM-assisted video content analysis, comparing AI's interpretations to human understanding of abstract concepts. We leverage LLaVA-1.6 Mistral 7B to interpret four abstract concepts regarding video-mediated self-disclosure, analyzing 725 keyframes from 142 depression-related YouTube short videos. We perform a qualitative analysis of MLLM's self-generated explanations and found that the degree of operationalization can influence MLLM's interpretations. Interestingly, greater detail does not necessarily increase human-AI alignment. We also identify other factors affecting AI alignment with human understanding, such as concept complexity and versatility of video genres. Our exploratory study highlights the need to customize prompts for specific concepts and calls for researchers to incorporate more human-centered evaluations when working with AI systems in a multimodal context.

==> premeable.tex <==
\usepackage{csquotes}
\makeatletter
\@ifclasswith{acmart}{anonymous}
{%
    % Usage: https://ctan.org/pkg/anonymous-acm
    \usepackage[true]{anonymous-acm}
}{%
    \usepackage[false]{anonymous-acm} 
}
\makeatother
\usepackage{ifdraft}
\usepackage{etoolbox} % for global bool
\usepackage{xspace}
\usepackage{color}
\usepackage{tabularray}
\usepackage{comment}
\usepackage{cleveref}
\renewcommand*{\cref}{\Cref}
\usepackage{hyphenat}
\usepackage{array}
\usepackage{booktabs}
\usepackage{tabularx} 
\usepackage{multirow}
\usepackage{longtable}
\usepackage{subfigure}
\usepackage{soul}
\usepackage{xcolor}
\usepackage{utfsym}%MnSymbol,utfsym,arev
\definecolor{lightyellow}{RGB}{255, 251, 204}

\usepackage{graphicx}
\usepackage{subcaption}


\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}


\usepackage{longtable}
\usepackage{colortbl}
\usepackage{multirow}
\usepackage{subcaption}
\usepackage{tabularray}
\usepackage{csquotes}

% Still need to single quote `like this' or \enquote*{like this}
\renewcommand{\mkblockquote}{\small\itshape}
\NewDocumentCommand{\pquote}{+O{} +m}{\blockquote[#1]{\textit{#2}}}

\newcommand{\elide}[1]{\textelp{}} % produces ... instead of argument
\NewDocumentCommand{\textrep}{+m +m}{\textins{#2}} 
% Usage: \textrep{a long quote}{this.} => [this.]
% Others:
% \textins{text} = [text]
% \textins*{T}ext = [T]ext
% text\textdel{s} = text[]
\settopmatter{printfolios=true}

\newcommand{\textcite}[1]{\citeauthor{#1}~\cite{#1}}

\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=.8pt] (char) {#1};}}
            
%\NewDocumentCommand{myhilight}{O{lightyellow} m}{%
%  \sethlcolor{#1}\hl{#2}%
%}

% annotations
\usepackage[textsize=scriptsize]{todonotes}
%\usepackage[textsize=scriptsize, disable]{todonotes}
\newcommand\sam[1]{\todo[color=blue!20]{{\bf Sam}: #1}}

%Color code
\definecolor{lightyellow}{RGB}{255, 251, 204}
\definecolor{lightgreen}{RGB}{204, 255, 204}

==> tabs/concepts.tex <==
\begin{table*}[h]
\caption{
% Four abstract visual concepts to explore MLLM understanding.
Four abstract visual concepts shaping video-mediated self-disclosure.
}
\label{tab:concepts}
\footnotesize
\begin{tblr}{
width = \textwidth,
colspec = {|Q[l,0.1]|Q[l,0.8]|},
hlines,
row{1} = {font=\bfseries,c,gray9},
}

Concept & Definition \\

Presenting & Presenting style involves the delivery of information, typically accompanied by visual aids like slides or graphics \cite{kelly-hedrick_its_2018}. \\
%& Does this picture communicate in a presenting style, yes or no? Explain your answer. 

Interacting & Interacting refers to creators establishing a simulated interpersonal relationship with their audience, fostering a sense of engagement and connection \cite{kelly-hedrick_its_2018}. \\
%& Does this picture portray an interacting style, yes or no? Explain your answer. 

Diversity & Diversity of an image includes varied scenes, color variation, compositional complexity, and originality of the image \cite{seckler2015linking}. \\
%& What level of diversity does this image communicate, low or high? Explain your answer. \\

%Emotional Valence & Emotional valence is the value associated with a stimulus as expressed on a continuum from pleasant to unpleasant or from attractive to aversive. & Is the emotional valence of the picture positive, negative, or neutral? Explain your answer. \\

Arousal & Arousal refers to the degree of alertness or excitement elicited by the stimulus such as dynamic visual elements and emotional intensity \cite{metallinos2013television}. \\
%& What level of arousal does this image communicate, low or high? Explain your answer. \\

\end{tblr}
\end{table*}


==> tabs/considerations.tex <==
\begin{table*}[h]
\caption{Considerations of prompt design}
\label{tab:considerations}
\small
\begin{tblr}{
width = \textwidth,
colspec = {|Q[l,0.15]|Q[l,0.5]|Q[l,0.3]|},
hlines,
row{1} = {font=\bfseries,c,gray9},
}

Categories & Definition & Example \\

Complexity of concepts & & \\

Opretionalization & & \\

Multimodal cues & & \\

\end{tblr}
\end{table*}


==> tabs/quant.tex <==
\begin{table*}[h]
\caption{Mean ± 2 * Std Accuracy Scores for Concepts and Prompt Strategies}
\label{tab:quant}
\footnotesize
\begin{tblr}{
  width = \textwidth,
  colspec = {|Q[c,0.18]|Q[c,0.15]|Q[c,0.15]|Q[c,0.15]|Q[c,0.15]|Q[c,0.15]|},
  hlines,
  row{1} = {font=\bfseries,c,gray9},
}
Prompt Strategy & Interacting & Presenting & Emotional Valence & Arousal & Diversity \\
Naive & 0.52 \pm 0.032 & 0.61 \pm 0.031 & 0.36 \pm 0.031 & 0.71 \pm 0.029 & 0.71 \pm 0.029 \\
Simple Definition & 0.45 \pm 0.032 & 0.63 \pm 0.031 & 0.36 \pm 0.031 & 0.72 \pm 0.028 & 0.73 \pm 0.028 \\
Detailed Definition & 0.53 \pm 0.032 & 0.56 \pm 0.031 & 0.3 \pm 0.029  & 0.71 \pm 0.029 & 0.74 \pm 0.027 \\
Openminded & 0.43 \pm 0.032 & 0.68 \pm 0.03  & 0.33 \pm 0.03  & 0.71 \pm 0.029 & 0.74 \pm 0.027 \\
\end{tblr}
\end{table*}

==> tabs/visualtask.tex <==
\begin{table*}[h]
\caption{Video Content Analysis Task Needs}
\label{tab:tasks}
\footnotesize
\begin{tblr}{
width = \textwidth,
colspec = {|Q[l,0.06]|Q[l,0.04]|Q[l,0.25]|Q[l,0.2]|},
hlines,
row{1} = {font=\bfseries,c,gray9},
}
Task Category & Task & Description & Examples \\
\SetCell[r=3]{m}{Identification} & Object & The presence or number of entities within the image, such as humans, objects, or animals are key to understanding the context of the video. & Presence of timer, number of people, presence of face in study livestream \cite{lee_personalizing_2021}  \\
%; Cultural heritage: ethnic minority language \cite{}
& Behavior& Identifying specific activities or actions the individuals or entities perform in the video. This helps categorize the video based on its dynamic elements. & Behaviors of eating, talking, and food preparation in Mukbang videos \cite{anjani_why_2020} \\ 
& Nuances & Details in the videos that contribute to the viewer's perception or comprehension of subtle elements. & Quantity and variety of food and lighting style in Mukbang videos \cite{anjani_why_2020} \\ 
\SetCell[r=3]{m}{Interpretation} 
& Emotion & Emotional expressions represented in the video, conveyed through facial expressions, tone, or other emotional cues. & Valence (positive or negative emotions expressed in the video) \cite{huh_health_2014} \\ 
& Genre & The classification of videos based on their topic, style, or content category, allowing better organization and interpretation of the material. & Video genres such as lifestyle genre \cite{niu_stayhome_2021} and educational genre \cite{lee_personalizing_2021} \\
& Concept & High-level themes or abstract ideas communicated in the video, such as communication styles or social roles. & Attachment, social integration, reassurance, nurturance in Covid-19 companion videos \cite{niu_stayhome_2021} \\

\end{tblr}
\end{table*}


% \begin{table*}[h]
% \caption{Video Content Analysis Task Needs}
% \label{tab:tasks}
% \footnotesize
% \begin{tblr}{
% width = \textwidth,
% colspec = {|Q[l,0.06]|Q[l,0.06]|Q[l,0.2]|Q[l,0.2]|},
% hlines,
% row{1} = {font=\bfseries,c,gray9},
% }
% Task Category & Task & Description & Examples \\
% \SetCell[r=3]{m}{Identification} & Object &  the presence or number of entities within the image, such as humans and food & Online study room: timer, number of people, face, chat room \cite{lee_personalizing_2021};  Cultural heritage: ethnic minority language \cite{} \\
% & Behavior&  identifying specific activities or actions the individuals perform in the video.   & Muckbang videos: eating, talking, \cite{anjani_why_2020}\\ 
% & Nuances & Details in the videos  & Quantity and variety of food, creators' attractiveness \cite{anjani_why_2020}\\ 
% \SetCell[r=3]{m}{Interpretation} & Concept & high level themes such as communication styles & Covid-19 companion videos: attachment, social integration, reassurance of worth, guidance, nurturance \cite{niu_stayhome_2021} \\
% & Emotion & emotional expressions represented in the video & Valence \cite{} \\
% %Audio features & & background music \cite{anjani_why_2020, lee_personalizing_2021}\\
% & Genre & & topics of videos \cite{niu_stayhome_2021}, area of study \cite{lee_personalizing_2021} \\

% \end{tblr}
% \end{table*}

